A Manually Annotated Chinese Corpus for Non-task-oriented Dialogue Systems

This paper presents a large-scale corpus for non-task-oriented dialogue response selection, which contains over 27K distinct prompts more than 82K responses collected from social media. To annotate this corpus, we define a 5-grade rating scheme: bad, mediocre, acceptable, good, and excellent, according to the relevance, coherence, informativeness, interestingness, and the potential to move a conversation forward. To test the validity and usefulness of the produced corpus, we compare various unsupervised and supervised models for response selection. Experimental results confirm that the proposed corpus is helpful in training response selection models.

==> intro-example.tex <==
\begin{table}\small
\centering
\begin{tabular}{|l|}
\hline
\textbf{Prompt}: Hey, Beijing, I'm coming!\\
\hline
\hline
\underline{\textbf{Unacceptable responses:}}\\
$[$R$_1]$: $<$\textsf{Nonsense}$>$ ddddd\\
$[$R$_2]$: $<$\textsf{Irrelevant}$>$ Maybe not?\\
$[$R$_3$: $<$\textsf{Incoherent}$>$ Beijing is larger than Shanghai.\\
$[$R$_4]$: $<$\textsf{Echoing}$>$ Beijing\\
\hline
\hline
\underline{\textbf{Marginally acceptable  responses:}}\\
$[$R$_5]$: $<$\textsf{General}$>$ Great!\\
$[$R$_6]$: $<$\textsf{ST-limited}$>$ Keep warm! It's snowing.\\
\hline
\hline
\underline{\textbf{Acceptable responses:}}\\
$[$R$_7]$: $<$\textsf{Good}$>$ Enjoy! Beijing is beautiful.\\
$[$R$_8]$: $<$\textsf{Excellent}$>$: Which hotel are you staying there?\\
 \hline
\end{tabular}
\caption{Different types of responses for ``\textit{Hey, Beijing, I'm coming!}''. $[$R$_i]$: the $i$-th user-generated response for the prompt post. $<$\textsf{Type}$>$: Human annotated types for responses regarding their quality as training data, where \textsf{ST-limited} refers to spatial or temporal limited.}\label{tab:intro-example}
\end{table}
